Benchmarking neural embeddings for link prediction in knowledge graphs under semantic and structural changes

Recently, link prediction algorithms based on neural embeddings have gained tremendous popularity in the Semantic Web community, and are extensively used for knowledge graph completion. While algorithmic advances have strongly focused on efficient ways of learning embeddings, fewer attention has been drawn to the different ways their performance and robustness can be evaluated. In this work we propose an open-source evaluation pipeline, which benchmarks the accuracy of neural embeddings in situations where knowledge graphs may experience semantic and structural changes. We define relation-centric connectivity measures that allow us to connect the link prediction capacity to the structure of the knowledge graph. Such an evaluation pipeline is especially important to simulate the accuracy of embeddings for knowledge graphs that are expected to be frequently updated.

==> sections/discussion.tex <==
\section{Discussion} \label{sec:discussion}
%
% \subsection{Related work}
% The most focused study of the link prediction problem for the large scale (unlabelled) graph-based data mining has been conducted in~\cite{garciagasulla_2016}, to the
% best of our knowledge. The focus of that work is on negative sample generation, and the author emphasize that the link prediction problem is a hugely imbalanced binary
% prediction task, where the number of negative samples is orders of magnitude higher than the number of positive examples. 
% % The solution presented is to use the constrained
% % ROC AUC evaluation metric, where the area under the false positive to true positive curve is proposed to be evaluated under a certain threshold. This threshold is
% % set to where the false positive rate reaches the true positive rate, i.e., when the classifier has accepted as many false negatives as there are true positives.
% In the bioinformatics community Alshahrani et al.~\cite{alshahrani_2017} proposed to circumvent the problem of imbalanced classes for the binary classification problem by
% considering negative links that have a biological meaning, truncating thus many potential negative links that are highly improbable biologically. They do this by
% restricting all the negative links to have the same domain and range as the positive links (i.e., they do not consider highly improbable links of type $gene_i$
% \textsc{has function} $drug_j, drug_j \not \in range(\text{\textsc{has function}})$). Link prediction for the entire knowledge graph is then treated as a set of binary
% classification tasks (one for each relation). Both of these works agree that link prediction should be treated as a binary classification task. 
% Some works have focused their attention on the strategies for data splitting, producing biased train and test examples, such that the implicit information from the test
% set may leak into the train set~\cite{toutanova_2016,dettmers_2017}. In~\cite{dettmers_2017}, authors show that the random splits for the common knowledge graph
% evaluation benchmarks (Wordnet~\cite{miller_1995} and Freebase~\cite{bollacker_2008}) may bias the classification results for the symmetric relations. Solutions to
% unbiased evaluations include curated data splits where no such information leakage is present. Kadlec et al.~\cite{kadlec_2017} have mentioned that fair optimization of
% hyperparameters for competing approaches should be considered, as some of the reported KG completion results are significantly lower than what they potentially could be.
% Evaluation of the machine learning tasks that use link information from the knowledge graphs and neural embeddings is explored in~\cite{ristoski_2016,cochez_2017}.
% 
% As a general remark, in most of the works, link prediction is evaluated with the mean rank metric and its variants from the information retrieval community  (e.g., mean
% reciprocal rank, top $k$ results, mean average precision), which we believe is not the most suitable metric for link prediction. As we pointed out in
% Section~\ref{sec:intro-lp}, the probability to have a new link $(e_i, r_i, e_j)$ is different from asking if the entity $e_j$ is part of the set of the most probable
% entities, among all existing entities in the knowledge graph, to be connected to $e_i$ with the relation $r_i$.
% 
% We believe that the evaluation of the quality of the embeddings for the link prediction task has received much less attention than the methodologies for training the
% embeddings in the literature. While most of the works do perform extensive evaluation of their embedding approaches, the exact steps and implications of negative sample
% generation, random train and test data splits, amount of information involved in the unsupervised learning, are either not very well detailed for an easy and fair
% reproducibility of the results, or are presented as a secondary remark.
% 

\subsection{Neural embedding model complexity}

The focus of our study has not been on obtaining best classification performance, but rather, supporting statistically and empirically the hypothesis, that the cheaper
and more scalable generalized embeddings can attain a similar performance as the more expensive specialized embeddings. In doing so, we sought to use a simpler neural
embedding model for faster, more scalable and broader evaluation of our results. The neural embedding model we use is a model that is shallow, in the number of model
parameters (e.g., number of hidden layers), and first-order, in terms of how much neighborhood information is used. More complex models with deeper and more sophisticated
architectures (i.e., involving more fully-connected and/or convolutional hidden layers~\cite{dettmers_2017,goyal_2018}), and/or models taking into account higher order
neighborhood information (i.e., models based on random walks~\cite{perozzi_2014,alshahrani_2017}, and/or based on graph depth traversal~\cite{grover_2016}) have not been
considered in this work. These models most likely would yield superior classification results. However, we have not investigated the convergence of the overall
performance distributions of specialized and generalized embeddings, trained with these models, due to increased complexity (time-wise) for statistical evaluations. Such
an evaluation could, however, benefit the community to analyze the behavior of more complex neural embedding models.

\subsubsection{Hyperparameter search}

While we report our statistical evaluation only for a fixed set of hyperparameters for the neural embedding model, we did experiment with different setting of the
hyperparameters. In particular, we experimented with the different dimension sizes ($d={5,10,20,50,100,512}$), and with the different number of epochs ($e={5,10,20,50}$)
for a smaller number of validation runs, and on medium-sized knowledge graphs only. In general, only slight improvements on the classification performance were observed.
Convergence of distributions for specialized and generalized embeddings being our primary target, we decided to perform full-scale statistical evaluation with the chosen
fixed set of hyperparameters ($d=50, e=10$).

\subsection{Link prediction} 

\subsubsection{Link representation or node combination}

Based on the embeddings of the nodes of the graph, we can come up with different ways of representing a link between an entity $e_i$ and $e_j$.  This is usually achieved
with a binary operator (or a node combination strategy) that transforms entity embeddings representations $\gamma(e_i), \gamma(e_j)$ into one single representation of the
link $(e_i, r_i, e_j)$.  Popular choices for this operator include operations that preserve the original $d$ dimension of the entity embeddings to represent links (e.g.,
element-wise sum or mean~\cite{grover_2016}), as well as the operations that concatenate entity embeddings~\cite{dettmers_2017,crichton_2018,agibetov_semdeep_2018}. In
our experiments with 10 cross-validation runs for the WN11 we observed that the concatenation operator outperformed other considered binary operators, and that all the
considered node combination strategies resulted in the convergence of performance distributions for specialized and generalized embeddings~\cite{agibetov_semdeep_2018}.
In this work we thus stuck with the concatenation as our binary operator for a broader evaluation with additional datasets. Using different node combination strategies on
different knowledge graphs, may or may not have significant impact on the performance.

\subsubsection{Negative sampling} \label{sec:neg-sampling}

In general, the link prediction problem for knowledge graphs is different from other classification problems where positive and negative examples are well defined, and
the \emph{iid} (independent and identically distributed random variables) assumption is valid. Obtaining a representative test set with a prototypical distribution is
often not trivial~\cite{garciagasulla_2016}, and usually what is done is that we randomly remove some links which we then use as our test positives (knowledge graph
completion under close-world assumption). Moreover, during the generation of negative links both for train and test sets, we impose that no negative link appears as a
training positive or test positive. We therefore implicitly leak information about the test positives when we generate train negatives. In other words, during the
generation of negative links $(\bar{e_i}, r_i, \bar{e_j}) \not \in Pos_{KG})$ we should account to the possibility that this link might actually turn out to be true, and
our binary classifiers should be robust and generalize well to these realistic situations. In our preliminary investigations on the impact of this bias we have not seen
big discrepancies in the classifiers' performance, however, a more elaborate analysis into this issue would be very interesting to the community.

%As our future work we would like to study further the implications of the negative example generation.

\subsection{Properties of knowledge graphs}

In our experiments we considered \emph{relation-centric} metrics $\phi(KG), \mu_{r_i}$ and $z_{r_i}$ to characterize the knowledge graphs. In particular, we used
$\mu_{r_i}$ and $z_{r_i}$ to identify the correlations of classifier performances, and studied the impact of \emph{multi-relationness} $\phi(KG)$ on overall classifier
performance. While we showed that they help identify the use-cases when the generalized embeddings perform almost identical on average as the specialized embeddings,
other characterizations of knowledge graph may better explain other trends. For instance, we have not observed conclusive correlations of \emph{relation-centric} metrics
with the ratio of missing examples at train/test phases. Perhaps \emph{entity-centric} metrics (e.g., incoming and/or outcoming node degree, PageRank centrality) might be
more suitable characterization metrics to explain to predict the missing ratios.

